Renormalized perturbation theory at large expansion orders

We present a general formalism that allows for the computation of large-order renormalized expansions in the spacetime representation, effectively doubling the numerically attainable perturbation order of renormalized Feynman diagrams. We show that this formulation compares advantageously to the currently standard techniques due to its high efficiency, simplicity, and broad range of applicability. Our formalism permits to easily complement perturbation theory with non-perturbative information, which we illustrate by implementing expansions renormalized by the addition of a gap or the inclusion of Dynamical Mean-Field Theory. As a result, we present numerically-exact results for the square-lattice Fermi-Hubbard model in the low temperature non-Fermi-liquid regime and show the momentum-dependent suppression of fermionic excitations in the antinodal region.

==> figure_spectral_functions.tex <==
\begin{figure}
  \includegraphics[width=0.5\textwidth]{spectral_function} 
  \caption{BETA 10:::::Partial sums for the average of number of particle per site, as a function of truncation order.  \label{Fig_density_beta10}}
\end{figure}


==> footnote_linear_renormalization.tex <==
\footnote{Renormalization schemes linear in the interaction do not give frequency-momentum dependence in the Hubbard model, and are therefore too limited for our purposes.}


==> footnote_rpa_det.tex <==
\footnote{RPA-DET}


==> intro_old.tex <==
Renormalization is one of the most fruitful ideas in physics. Originally discovered as a trick to get rid of one-loop Feynman-diagram infinities in quantum electrodynamics~\cite{qed_bethe, qed_tomonaga, qed_feynman, qed_schwinger}, it has lead to one of the most precise comparison of theory and experiments~\cite{qed_exp_th}. It was later understood that renormalization is useful way beyond high-energy physics, and it was applied to condensed matter physics~\cite{abrikosov_book} and especially to the theory of critical phenomena~\cite{wilson_epsilon_expansion}, leading to the development of the perturbative renormalization group techniques. Computing renormalized Feynman diagrams is therefore at the core of our quantitative understanding of nature, and it is therefore important to find efficient strategies to perform this computation. Evaluating a large number of diagram loops  is an extremely challenging task even with modern computational facilities. For example, no 6-loop QED computation has ever been attempted, despite its experimental interest. The reason for this limitation is that Feynman diagram computations are limited by the ``factorial barrier'' represented by the explosion of the number of diagrams with increasing number of loops. Diagrammatic Monte Carlo techniques~\cite{prokofiev_svistunov, kris_felix, deng} were introduced with the idea that Feynman diagrams could be good sampling variables in strongly-correlated electronic systems as they can be defined directly in the thermodynamic limit and continuum limit.  While they dramatically simplified and automatized the computation of Feynman diagrams, and there are many recent advancements in this direction~\cite{kun_chen}, they are still limited by the factorial barrier as they consider explicit Feynman diagram topologies.


==> paragraph_extensions.tex <==
SKETCH: This work can be extended to the renormalization of vertex functions. We can get more physics. We can do continuum limit, and electron gas. 


==> quadratic_renormalization.tex <==
\begin{figure}
  \includegraphics[width=0.5\textwidth]{diagrams}
\caption{Top: Dyson-like equation defining the bare Green's function $G_0$, the renormalized Green's function $G_R$ and the second order shift $\Sigma_R$. Bottom: explicit examples of diagrams contributing to the physical Green's function $G$. \label{Fig_Hubbard_atom}}
\end{figure}



==> sentence_bold_kfg.tex <==
The problem with the first approach is that it has been found that the bold scheme can converge towards an unphysical answer at strong interaction~\cite{kfg}.


==> sentence_complexity_shift.tex <==
We want to stress that the complexity of the computation is independent of the complexity of the shift.


==> sentence_superfluid_instability.tex <==
Moreover, the presence of the superfluid instability in  the attractive model at $U<0$ shrinks the radius of convergence of the series to zero at zero temperature.

